Approximating Numerical Fluxes Using Fourier Neural Operators for Hyperbolic Conservation Laws

Traditionally, classical numerical schemes have been employed to solve partial differential equations (PDEs) using computational methods. Recently, neural network-based methods have emerged. Despite these advancements, neural network-based methods, such as physics-informed neural networks (PINNs) and neural operators, exhibit deficiencies in robustness and generalization. To address these issues, numerous studies have integrated classical numerical frameworks with machine learning techniques, incorporating neural networks into parts of traditional numerical methods. In this study, we focus on hyperbolic conservation laws by replacing traditional numerical fluxes with neural operators. To this end, we developed loss functions inspired by established numerical schemes related to conservation laws and approximated numerical fluxes using Fourier neural operators (FNOs). Our experiments demonstrated that our approach combines the strengths of both traditional numerical schemes and FNOs, outperforming standard FNO methods in several respects. For instance, we demonstrate that our method is robust, has resolution invariance, and is feasible as a data-driven method. In particular, our method can make continuous predictions over time and exhibits superior generalization capabilities with out-of-distribution (OOD) samples, which are challenges that existing neural operator methods encounter.

==> FNO <==
\begin{thebibliography}{42}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi: #1}\else
  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi

\bibitem[Basir and Senocak(2022)]{Basir:20}
S.~Basir and I.~Senocak.
\newblock Critical investigation of failure modes in physics-informed neural networks.
\newblock \emph{AiAA SCITECH 2022 Forum}, 2022.

\bibitem[Benitez et~al.(2023)Benitez, Furuya, Faucher, Kratsios, Tricoche, and Hoop]{Benitez:23}
J.A.L. Benitez, T.~Furuya, F.~Faucher, A.~Kratsios, X.~Tricoche, and M.V.D Hoop.
\newblock Out-of-distributional risk bounds for neural operators with applications to the helmholtz equation.
\newblock \emph{arXiv}, arXiv:2301.11509, 2023.

\bibitem[Cai et~al.(2021)Cai, Chen, and Liu]{Cai:21}
Z.~Cai, J.~Chen, and M.~Liu.
\newblock Least-squares relu neural network (lsnn) method for linear advection-reaction equation.
\newblock \emph{Journal of Computational Physics}, 443:\penalty0 686--707, 2021.

\bibitem[Chen et~al.(2022)Chen, Gelb, and Lee]{Chen:22}
Z.~Chen, A.~Gelb, and Y.~Lee.
\newblock Designing neural networks for hyperbolic conservation laws.
\newblock \emph{arXiv}, arXiv:2211.14375, 2022.

\bibitem[Courant et~al.(1952)Courant, Isaacson, and Rees]{Courant:52}
R.~Courant, E.~Isaacson, and M.~Rees.
\newblock On the solution of nonlinear hyperbolic differential equations by finite differences.
\newblock \emph{Communications on Pure and Applied Mathematics}, 5\penalty0 (3):\penalty0 243--255, 1952.

\bibitem[Fu(2019)]{Fu:19}
L.~Fu.
\newblock A very-high-order teno scheme for all-speed gas dynamics and turbulence.
\newblock \emph{Computer Physics Communications}, 244:\penalty0 117--131, 2019.

\bibitem[G.~Gupta and Bogdan(2021)]{Gupta:21}
X.~Xiao G.~Gupta and P.~Bogdan.
\newblock Multiwavelet-based operator learning for differential equations.
\newblock \emph{Advances in Neural Information Processing Systems}, 2021.

\bibitem[Godunov(1959)]{Godunov:59}
S.K. Godunov.
\newblock A difference method for numerical calculation of discontinuous solutions of the equations of hydrodynamics.
\newblock \emph{Matematicheskii Sbornik}, 47\penalty0 (3):\penalty0 271--306, 1959.

\bibitem[Gopalani et~al.(2022)Gopalani, Karmakar, and Mukherjee]{Gopalani:22}
P.~Gopalani, S.~Karmakar, and A.~Mukherjee.
\newblock Capacity bounds for the deeponet method of solving differential equations.
\newblock \emph{arXiv}, arXiv:2205.11359, 2022.

\bibitem[Gottlieb and Shu(1998)]{Gottlieb:98}
S.~Gottlieb and C.W. Shu.
\newblock Total variation diminishing runge-kutta schemes.
\newblock \emph{Mathematics of Computation}, 67:\penalty0 73--85, 1998.

\bibitem[Harten et~al.(1987)Harten, Engquist, Osher, and Chakravarthy]{Harten:87}
A.~Harten, B.~Engquist, S.~Osher, and S.~Chakravarthy.
\newblock Uniformly high order essentially non- oscillatory schemes iii.
\newblock \emph{Journal of Computational Physics}, 71\penalty0 (2):\penalty0 231--303, 1987.

\bibitem[Holl et~al.(2020)Holl, Koltun, and Thuerey]{Holl:20}
P.~Holl, V.~Koltun, and N.~Thuerey.
\newblock Learning to control pdes with differentiable physics.
\newblock \emph{ICLR 2020}, 2020.

\bibitem[Jakubovitz et~al.(2019)Jakubovitz, Giryes, and Rodrigues]{Jaku:19}
D.~Jakubovitz, R.~Giryes, and M.R.D. Rodrigues.
\newblock \emph{Generalization Error in Deep Learning}.
\newblock Birkhäuser Cham, 2019.

\bibitem[Jin(1995)]{Jin:95}
S.~Jin.
\newblock Runge-kutta methods for hyperbolic conservation laws with stiff relaxation terms.
\newblock \emph{Journal of Computational Physics}, 122\penalty0 (1):\penalty0 51--67, 1995.

\bibitem[Kim and Kang(2024)]{Kim:24}
T.~Kim and M.~Kang.
\newblock Bounding the rademacher complexity of fourier neural operators.
\newblock \emph{Machine Learning}, 113, 2024.

\bibitem[Kossaczká et~al.(2021)Kossaczká, Ehrhardt, and Günther]{Kossaczka:21}
T.~Kossaczká, M.~Ehrhardt, and M.~Günther.
\newblock Enhanced fifth order weno shock-capturing schemes with deep learning.
\newblock \emph{Results in Applied Mathematics}, 12\penalty0 (100201), 2021.

\bibitem[Kovachki et~al.(2021{\natexlab{a}})Kovachki, Lanthaler, and Mishra]{Kovachki:21}
N.~Kovachki, S.~Lanthaler, and S.~Mishra.
\newblock On universal approximation and error bounds for fourier neural operators.
\newblock \emph{Journal of Machine Learning Research}, 22\penalty0 (290), 2021{\natexlab{a}}.

\bibitem[Kovachki et~al.(2021{\natexlab{b}})Kovachki, Li, Liu, Azizzadenesheli, Bhattacharya, Stuart, and Anandkumar]{Kovachki:212}
N.~Kovachki, Z.~Li, B.~Liu, K.~Azizzadenesheli, K.~Bhattacharya, A.~Stuart, and A.~Anandkumar.
\newblock Neural operator: Learning maps between function spaces.
\newblock \emph{arXiv}, arXiv:2108.08481, 2021{\natexlab{b}}.

\bibitem[Lax(1954)]{Lax:54}
P.D. Lax.
\newblock Weak solutions of nonlinear hyperbolic equations and their numerical computation.
\newblock \emph{Communications on Pure and Applied Mathematics}, 7\penalty0 (1):\penalty0 159--193, 1954.

\bibitem[Leer(1974)]{Leer:74}
B.V. Leer.
\newblock Towards the ultimate conservative difference scheme. ii. monotonicity and conservation combined in a second-order scheme.
\newblock \emph{Journal of Computational Physics}, 14\penalty0 (4):\penalty0 361--370, 1974.

\bibitem[LeVeque(1992)]{LeVeque:92}
R.J. LeVeque.
\newblock \emph{Numerical Methods for Conservation Laws}.
\newblock Birkhäuser Basel, 1992.

\bibitem[Li et~al.(2020)Li, Kovachki, Azizzadenesheli, Liu, Bhattacharya, Stuart, and Anandkumar]{Li:20}
Z.~Li, N.~Kovachki, K.~Azizzadenesheli, B.~Liu, K.~Bhattacharya, A.~Stuart, and A.~Anandkumar.
\newblock Neural operator: Graph kernel network for partial differential equations.
\newblock \emph{ICLR 2020 Workshop ODE/PDE+DL}, 2020.

\bibitem[Li et~al.(2021)Li, Kovachki, Azizzadenesheli, Liu, Bhattacharya, Stuart, and Anandkumar]{Li:21}
Z.~Li, N.~Kovachki, K.~Azizzadenesheli, B.~Liu, K.~Bhattacharya, A.~Stuart, and A.~Anandkumar.
\newblock Fourier neural operator for parametric partial differential equations.
\newblock \emph{ICLR 2021}, 2021.

\bibitem[Liu et~al.(1994)Liu, Osher, and Chan]{Liu:94}
X.D. Liu, S.~Osher, and T.~Chan.
\newblock Weighted essentially non-oscillatory schemes.
\newblock \emph{Journal of Computational Physics}, 115\penalty0 (1):\penalty0 200--212, 1994.

\bibitem[Lu et~al.(2021)Lu, Jin, Pang, Zhang, and Karniadakis]{Lu:21}
L.~Lu, P.~Jin, G.~Pang, Z.~Zhang, and G.E. Karniadakis.
\newblock Learning nonlinear operators via deeponet based on the universal approximation theorem of operators.
\newblock \emph{Nature Machine Intelligence}, 3\penalty0 (3):\penalty0 218--229, 2021.

\bibitem[Magier et~al.(2020)Magier, Ray, Hesthaven, and Rohde]{Magiera:20}
J.~Magier, D.~Ray, J.S. Hesthaven, and C.~Rohde.
\newblock Constraint-aware neural networks for riemann problems.
\newblock \emph{Journal of Computational Physics}, 409:\penalty0 109345, 2020.

\bibitem[Mojgani et~al.(2023)Mojgani, Balajewicz, and Hassanzadeh]{Mojgani:23}
R.~Mojgani, M.~Balajewicz, and P.~Hassanzadeh.
\newblock Kolmogorov n–width and lagrangian physics-informed neural networks: A causality-conforming manifold for convection-dominated pdes.
\newblock \emph{Computer Methods in Applied Mechanics and Engineering}, 404:\penalty0 115810, 2023.

\bibitem[O'Shea and Nash(2015)]{O'Shea:15}
K.~O'Shea and R.~Nash.
\newblock An introduction to convolutional neural networks.
\newblock \emph{arXiv}, arXiv:1511.08458, 2015.

\bibitem[Pathak et~al.(2022)Pathak, subramanian, Harrington, Raja, Chattopadhyay, Mardani, Kurth, Hall, Li, Azizzadenesheli, Hassanzadeh, Kashinath, and Anandkumar]{Pathak:22}
J.~Pathak, S~subramanian, P.~Harrington, S.~Raja, A.~Chattopadhyay, M.~Mardani, T.~Kurth, D.~Hall, Z.~Li, K.~Azizzadenesheli, P.~Hassanzadeh, K.~Kashinath, and A.~Anandkumar.
\newblock Fourcastnet: A global data-driven high-resolution weather model using adaptive fourier neural operators.
\newblock \emph{arXiv}, arXiv:2202.11214, 2022.

\bibitem[Ray and Hesthaven(2018)]{Ray:18}
D.~Ray and J.S. Hesthaven.
\newblock An artificial neural network as a troubled-cell indicator.
\newblock \emph{Journal of Computational Physics}, 367:\penalty0 166--191, 2018.

\bibitem[Ruggeri et~al.(2022)Ruggeri, Roy, Mueterthies, Gruenwald, and Scalo]{Ruggeri:22}
M.~Ruggeri, I.~Roy, M.J. Mueterthies, T.~Gruenwald, and C.~Scalo.
\newblock Neural-network-based riemann solver for real fluids and high explosives; application to computational fluid dynamics.
\newblock \emph{Physics of Fluids}, 34\penalty0 (11):\penalty0 116121, 2022.

\bibitem[Shahabi and Ghiassi(2022)]{Shahabi:22}
A.~Shahabi and R.~Ghiassi.
\newblock A robust second-order godunov-type method for burgers’ equation.
\newblock \emph{International Journal of Applied and Computational Mathematics}, 8\penalty0 (82), 2022.

\bibitem[Shalev-Shwartz and Ben-David(2014)]{shalev:88}
Shai Shalev-Shwartz and Shai Ben-David.
\newblock \emph{Understanding Machine Learning: From Theory to Algorithms}.
\newblock Cambridge University Press, San MateoShaftesbury Road, Cambridge, 2014.

\bibitem[Shu and Osher(1988)]{Shu:88}
C.W. Shu and S.~Osher.
\newblock Efficient implementation of essentially non-oscillatory shock- capturing schemes.
\newblock \emph{Journal of Computational Physics}, 21:\penalty0 439--471, 1988.

\bibitem[Sirignano and Spiliopoulos(2018)]{Sirignano:18}
J.~Sirignano and K.~Spiliopoulos.
\newblock Dgm: A deep learning algorithm for solving partial differential equations.
\newblock \emph{Journal of Computational Physics}, 375:\penalty0 1339--1364, 2018.

\bibitem[Sweby(1984)]{Sweby:84}
P.K. Sweby.
\newblock High resolution schemes using flux limiters for hyperbolic conservation laws.
\newblock \emph{SIAM journal on numerical analysis}, 21\penalty0 (5):\penalty0 995--1011, 1984.

\bibitem[Valiant(1984)]{Valiant:84}
L.G. Valiant.
\newblock A theory of the learnable.
\newblock \emph{Communications of the ACM}, 27\penalty0 (11):\penalty0 1134--1142, 1984.

\bibitem[Vapnik(1999)]{vapnik:21}
V.N. Vapnik.
\newblock An overview of statistical learning theory.
\newblock \emph{IEEE Transactions on Neural Networks}, 10\penalty0 (5):\penalty0 988--999, 1999.

\bibitem[Wang et~al.(2022)Wang, Yu, and Perdikaris]{Wang:22}
S.~Wang, X.~Yu, and P.~Perdikaris.
\newblock When and why pinns fail to train: A neural tangent kernel perspective.
\newblock \emph{Journal of Computational Physics}, 449:\penalty0 110768, 2022.

\bibitem[Wang et~al.(2020)Wang, Shen, Long, and Dong]{Wang:20}
Y.~Wang, Z.~Shen, Z.~Long, and B.~Dong.
\newblock Learning to discretize: Solving 1d scalar conservation laws via deep reinforcement learning.
\newblock \emph{arXiv}, arXiv:1905.11079, 2020.

\bibitem[Weinan and Yu(2018)]{Weinan:18}
E.~Weinan and B.~Yu.
\newblock The deep ritz method: A deep learning-based numerical algorithm for solving variational problems.
\newblock \emph{Communications in Mathematics and Statistics}, 6:\penalty0 1--12, 2018.

\bibitem[Wen et~al.(2022)Wen, Li, Azizzadenesheli, Anandkumar, and Benson]{Wen:22}
G.~Wen, Z.~Li, K.~Azizzadenesheli, A.~Anandkumar, and S.M. Benson.
\newblock U-fno—an enhanced fourier neural operator-based deep-learning model for multiphase flow.
\newblock \emph{Advances in Water Resources}, 163, 2022.

\end{thebibliography}

